RobustTAD: Robust Time Series Anomaly Detection via Decomposition and Convolutional Neural Networks

The monitoring and management of numerous and diverse time series data at Alibaba Group calls for an effective and scalable time series anomaly detection service. In this paper, we propose RobustTAD, a Robust Time series Anomaly Detection framework by integrating robust seasonal-trend decomposition and convolutional neural network for time series data. The seasonal-trend decomposition can effectively handle complicated patterns in time series, and meanwhile significantly simplifies the architecture of the neural network, which is an encoder-decoder architecture with skip connections. This architecture can effectively capture the multi-scale information from time series, which is very useful in anomaly detection. Due to the limited labeled data in time series anomaly detection, we systematically investigate data augmentation methods in both time and frequency domains. We also introduce label-based weight and value-based weight in the loss function by utilizing the unbalanced nature of the time series anomaly detection problem. Compared with the widely used forecasting-based anomaly detection algorithms, decomposition-based algorithms, traditional statistical algorithms, as well as recent neural network based algorithms, RobustTAD performs significantly better on public benchmark datasets. It is deployed as a public online service and widely adopted in different business scenarios at Alibaba Group.

==> backup-2-related-work-new.tex <==
\section{Related Work}

Anomaly detection has been researched for over a century~\cite{AD_survey_2009}.\textbf{(Research on anomaly detection has been around for over a century)} A detailed
survey of prior work is beyond the scope of this paper. Here we give a brief overview of the
major types of time series anomaly detection algorithms and some of the most recent 
developments. 




% \subsection{Related Work}

One of the straightforward methods for time series anomaly detection is
to apply forecasting algorithms directly. In forecasting-based anomaly detection 
methods, a predictive model is first learned 
based on the historical data, which can predict the future observation based 
on the past history. 
% Formally, assume we first build a forecasting model which uses the most recent $w$
observations to predict the observation following them. When the newest observation
$y_t$ comes, we can use the history $y_{t-w}, \cdots, y_{t-2}, y_{t-1}$ and the forecasting
model to predict $y_t$ (we denote the predication as $\hat{y}_t$). Then we can compare $y_t$
with $\hat{y}_t$ to determine $y_t$ is anomaly if their difference is significant.

The forecasting based models can be divided into two categories. The first category is based on
traditional time series analysis in statistics. Typical examples include ARIMA (and its variants)~\cite{forecasting:book}, 
State Space Models (SSM)~\cite{SSM:book}, and Holt-Winters method~\cite{forecasting:book}. Due to their
simplicity and decent performance, these forecasting algorithms based on time series analysis
still attracts a lot of attentions in both industry and academy. \textbf{(delete on?)}

The second category is machine learning based methods. These methods cast the forecasting problem
as a supervised learning problem. As a result, many existing supervised learning algorithms, including 
deep neural network~\cite{deep:learning:book}, gradient boosting decision tree~\cite{hastie:book}, can be applied directly.

One of the advantages of forecasting-based anomaly detection methods is that many existing forecasting 
algorithms can be borrowed directly. However, many of them are not robust
to noises or outliers.  Note that almost all forecasting models essentially estimates a reference value $\hat{x}_t$ to determine 
whether $x_t$ is an outlier. \textbf{(should we use y_t as before)} However, this reference value is achieved by building a forecasting 
model. We argue that this process is\textbf{{may be?}} over-modeling since the estimation of the reference value
can be done in a more direct and efficient way. Furthermore, we cannot distinguish different types 
of anomalies by applying forecasting models directly. Also when 
data comes as a stream, the predictive model updating is required, which may be prohibitive for many models. \textbf{(prohibitive?)}

Another challenge in time series anomaly detection is how to 
remove the seasonality component as it is commonly observed
in many real-world data. In fact, many seasonal adjustment decompositions have been proposed in the literature~\cite{STL_cleveland1990stl,MSTL_hyndman2018package,STR_dokumentov2015str,TBATS_de2011forecasting,twitter:anomaly:detection,AD_laptev2015generic,X13ARIMA}. 

The most classical and widely used decomposition method is the STL
(Seasonal-Trend decomposition using Loess)~\cite{STL_cleveland1990stl} decomposition. 
In STL, the trend and seasonality components are estimated by using an alternating
algorithm where the trend component is computed using LOESS (LOcal regrESSion) smoothing. 
To handle multiple seasonalities, an extension called MSTL~\cite{MSTL_hyndman2018package} 
has been proposed recently.  
Its framework is similar to STL, and the difference lies in how to estimate multiple 
seasonality components, which are also estimated iteratively by fixing trend and rest 
seasonality components in MSTL. 
However, STL and MSTL fails to extract the seasonality component accurately 
when seasonality shift and fluctuation exist. 

Some recent decompositions include STR and TBATS. 
In \cite{STR_dokumentov2015str}, a Seasonal-Trend decomposition 
procedure based on Regression (STR) is proposed. In STR, 
a two-dimensional representation
of the seasonality component is utilized to learn the slowly
changing seasonality component. STR is flexible to seasonal 
shift and can deal with multiple seasonalities. Unfortunately, it cannot
scale to time series with long seasonality period due to the
cost to learn the huge two-dimensional structure. 

In TBATS (Trigonometric Exponential Smoothing
State Space model with Box-Cox transformation, ARMA errors,
Trend and Seasonal Components)~\cite{TBATS_de2011forecasting}, a 
framework based on state space model is introduced for complex
seasonal time series with multiple seasonal periods, high frequency
seasonality and non-integer seasonality. It incorporates Box-Cox
transformations, Fourier representations, and ARMA error correlation. 
Although an efficient method is proposed to estimate the parameters 
of the state space model, parameter estimation is still a burden 
especially when the seasonality period is long. Also \textbf{(In addition,)}
it cannot handle abrupt change of trend. 

We note that some prior work on decomposition-based anomaly detection. \textbf{(sounds bit strange)}
In ~\cite{twitter:anomaly:detection}, Seasonal ESD (S-ESD) and Seasonal Hybrid ESD (S-H-ESD)
have been proposed based on the practice at Twitter. 
Both algorithms employ the standard STL decomposition to remove 
the seasonal component and apply Extreme Studentized Deviate (ESD) test to identify
most significant anomalies. Compared with S-ESD, S-H-ESD applied median and 
median absolute deviation (MAD) in ESD to make it more robust to outliers. Unfortunately, 
both algorithms can only handle spike and dip anomalies, and the use of the 
standard STL makes it fail to deal with seasonality shift and fluctuation. 
